CSGO: Constrained-Softassign Gradient Optimization For Large Graph Matching

Graph matching aims to find correspondences between two graphs. This paper integrates several well-known graph matching algorithms into a framework: the constrained gradient method. The primary difference among these algorithms lies in tuning a step size parameter and constraining operators. By leveraging these insights, we propose an adaptive step size parameter to guarantee the underlying algorithms' convergence, simultaneously enhancing their efficiency and robustness. For the constraining operator, we introduce a scalable softassign for large graph matching problems. Compared to the original softassign, our approach offers increased speed, improved robustness, and reduced risk of overflow. The advanced constraining operator enables a CSGO for large graph matching, which outperforms state-of-the-art methods in experiments. Notably, in attributed graph matching tasks, CSGO achieves an over 10X increase in speed compared to current constrained gradient algorithms.

==> General_iterative_formula.tex <==
\section{Restricted gradient method}
In this section, we first recall a relaxation method, which transforms the discrete problem into a continuous one. Then, we introduce the projected fixed-point method to solve the doubly stochastic relaxed form of problem \eqref{eq.Object_fast}. 
%RRWN\cite{2010Reweighted},

\subsection{Relaxation method}
Due to the discrete constraints, \eqref{eq.Object_fast}  is an NP-hard problem. A common technique to solve this is first to solve a relaxed form of the discrete problem, whose solution is easy to obtain. Then the solution is converted back into the initial discrete domain by discrete projection schemes introduced in section 4. 
By relaxing the integer constraints from problem \eqref{eq.Object_fast}, a continuous problem with doubly stochastic constraints can be obtained:
\begin{equation}
\max _{{M}}\quad \frac{1}{2} \operatorname{tr}\left({M}^{T} {A} {M} {\widetilde{A}}\right)+\lambda \operatorname{tr}\left({M}^{T}{K}\right), \ \ \  \mathbf{M}\in \Sigma_{n \times n},
\label{eq.Object_relaxedKB}
\end{equation}
where $\Sigma_{n \times n} :=\{\mathbf{M}: \mathbf{M}\mathbf{1}=\mathbf{1},\mathbf{M}^{T}\mathbf{1}=\mathbf{1}, \mathbf{M} \geq 0$\} is the convex hull of $\Pi_{n \times n}$.
The relaxed constraints require $M$ to be a \textit{doubly stochastic matrix}.

We note that in spectral matching \cite{leordeanu2005spectral}, a more relaxed constraint $M \geq 0$ is used. Though fewer constraints can simplify the problem, accuracy of matching may decrease.



 \subsection{Projected fixed-point method}
For problem \eqref{eq.Object_relaxedKB}, some popular graph matching methods, such as SM, GA, IPFP, and DSPFP, can be unified into the same framework:

\begin{equation}
\begin{array}{cc}

    M^{(k+1)}=(1- \alpha)M^{(k)}  + \alpha D^{(k)} ,\\
    D^{(k)} = \mathcal{P}(\nabla Z) = \mathcal{P}(AM^{(k)}\tilde{A}+\lambda K).
    \end{array}
    \label{iter.DSPFP}
\end{equation}
Here $\mathcal{P}$ is a general projection/restriction operator which depends on the underlying constraints. The constraints manifest themselves in the projection scheme and the step size parameter. The computational cost of each iteration is $O(n^3)$. A fast projected fixed-point framework is shown in Algorithm \ref{ag.pfp}.


\begin{CJK*}{UTF8}{gkai}
    \begin{algorithm}
        \caption{ $\,$  Fast Projected Fixed-Point Framework}
        \begin{algorithmic}[1] 
            \Require $A,\tilde{A},K,\lambda,\alpha$
            \Ensure $M$       
                 \State $Initial$  $N$
                 \While{N does not converge \textbf{or} $iterations<I_1$}
                    \State $N =(1-\alpha)N+\alpha \mathcal{P}(AN \tilde{A}+\lambda K$)
                \EndWhile
                \State $Discretize$ $N$ $to$ $obtain$ $M$
                \State \Return{$M$}

        \end{algorithmic}
        \label{ag.pfp}
    \end{algorithm}
\end{CJK*}

The iterative formula can be converted into a more general form for relaxed problem \eqref{eq.IQP}: 
\begin{equation}
\begin{array}{cc}

    m^{(k+1)}=(1- \alpha)m^{(k)}  + \alpha d^{(k)},\\
    d^{(k)} = \mathcal{P}(\nabla z)  = \mathcal{P}(Wm +\lambda k) = \mathcal{P}(\operatorname{vec}{(\nabla Z)}).
    \end{array}
    \label{iter.quadratic}
\end{equation}
However, the computational cost of each iteration increases to $O(n^4)$. The SM, GA, and IPFP all share this form. 


%Correspondingly, their projection sets are subsets of the constraints sets respectively.

% $\arg \max _{\alpha} f\left((1-\alpha) m^{(k)}+\alpha d^{(k)}\right)$

% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \begin{table}[]
% \centering
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{ccccc}
% \multicolumn{5}{c}{\textbf{Summary of algorithms based on projected fixed-point framework}}                   \\ \hline
% \multicolumn{1}{l}{}      & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{}                            & \multicolumn{1}{l}{} \\
% Methods                         & Constraints         & Step size & $d^{(k)}$       & Cost/iteration \\
% SM\cite{leordeanu2005spectral}  & $m \in \mathscr{O}$ & 1         & $P_N(\nabla f)$ & $O(n^4)$       \\
% RRWN\cite{2010Reweighted} & $m \in \mathscr{O}$  & 1                    & $\theta P_N(\nabla f)+ (1-\theta)P_S(\nabla f)$ & 1                    \\
% GA\cite{gold1996graduated}      & $m \in \mathscr{d}$ & 1         & $P_S(\nabla f)$ & 1              \\
% IPFP\cite{leordeanu2009integer} & $m \in \mathscr{d}$ & adaptive  & $P_H(\nabla f)$ & 1              \\
% DSPFP\cite{lu2016fast}          & $M \in \mathscr{D}$ & 0.5       & $P_D(\nabla f)$ & 1             
% \end{tabular}%
% }
% \end{table}

% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
